AGN STORM 2: IX. Studying the Dynamics of the Ionized Obscurer in Mrk 817 with High-resolution X-ray Spectroscopy

We present the results of the XMM-Newton and NuSTAR observations taken as part of the ongoing, intensive multi-wavelength monitoring program of the Seyfert 1 galaxy Mrk 817 by the AGN Space Telescope and Optical Reverberation Mapping 2 (AGN STORM 2) Project. The campaign revealed an unexpected and transient obscuring outflow, never before seen in this source. Of our four XMM-Newton/NuSTAR epochs, one fortuitously taken during a bright X-ray state has strong narrow absorption lines in the high-resolution grating spectra. From these absorption features, we determine that the obscurer is in fact a multi-phase ionized wind with an outflow velocity of $\sim$5200 km s$^{-1}$, and for the first time find evidence for a lower ionization component with the same velocity observed in absorption features in the contemporaneous HST spectra. This indicates that the UV absorption troughs may be due to dense clumps embedded in diffuse, higher ionization gas responsible for the X-ray absorption lines of the same velocity. We observe variability in the shape of the absorption lines on timescales of hours, placing the variable component at roughly 1000 $R_g$ if attributed to transverse motion along the line of sight. This estimate aligns with independent UV measurements of the distance to the obscurer suggesting an accretion disk wind at the inner broad line region. We estimate that it takes roughly 200 days for the outflow to travel from the disk to our line of sight, consistent with the timescale of the outflow's column density variations throughout the campaign.

==> defns.tex <==
%\def\uveci{\ifmmode {\bf \hat{i}} \else {\bf i}\fi}
%\def\uvecj{\ifmmode {\bf j} \else {\bf j}\fi}
%\def\uveck{\ifmmode {\bf k} \else {\bf k}\fi}
%\def\uvecr{\ifmmode {\bf r} \else {\bf r}\fi}
%\def\vectorr{\makebox{\boldmath ${\bf r}$}}
\def\uveci{\makebox{\boldmath $\hat{\i}$}}
\def\uvecj{\makebox{\boldmath $\hat{\j}$}}
\def\uveck{\makebox{\boldmath $\hat{\rm k}$}}
\def\uvecr{\makebox{\boldmath $\hat{\rm r}$}}
\def\uvecth{\makebox{\boldmath $\hat{\theta}$}}
\def\vectora{\makebox{\bf a}}
\def\vectorr{\makebox{\bf r}}
\def\vectorL{\makebox{\bf L}}
\def\vectorp{\makebox{\bf p}}
\def\vectorv{\makebox{\bf v}}
\def\vectorF{\makebox{\bf F}}
\def\vectorC{\makebox{\bf C}}
\def\vectorB{\makebox{\bf B}}
\def\vectoromega{\makebox{\boldmath $\omega$}}
\def\vectoromegasid{\makebox{\boldmath $\omega_{\rm sid}$}}
\def\vectoromegasol{\makebox{\boldmath $\omega_{\rm sol}$}}
\def\vectoromegasyn{\makebox{\boldmath $\omega_{\rm syn}$}}
\def\vectortau{\makebox{\boldmath $\tau$}}
\def\vectoromegaE{\makebox{\boldmath $\omega_{\bf E}$}}
\def\vectoromegaP{\makebox{\boldmath $\omega_{\bf P}$}}
\def\vectoromegaS{\makebox{\boldmath $\omega_{\bf S}$}}
\def\vectoromegaMars{\makebox{\boldmath $\omega_{\bf Mars}$}}
%\newcommand{\degree}{\mbox{$^{\rm o}$}}
\newcommand{\degpoint}{\mbox{$^{\rm o}\!.$}}
\newcommand{\arcminpoint}{\mbox{$'\!.$}}
\newcommand{\arcsecpoint}{\mbox{$''\!.$}}
\newcommand{\marcsec}{\mbox{mas}}
\newcommand{\uas}{\mbox{$\mu$as}}
\newcommand{\parallax}{\mbox{$\pi''$}}
\newcommand{\kms}{\mbox{km\,s$^{-1}$}}
\newcommand{\pc}{\mbox{pc}}
\newcommand{\AU}{\mbox{AU}}
\newcommand{\dex}{\mbox{dex}}
%\newcommand{\cm2}{\mbox{cm$^{2}$}}
\newcommand{\cc}{\mbox{cm$^{-3}$}}
\newcommand{\kgm}{\mbox{kg\,m$^{-3}$}}
\newcommand{\Mearth}{\mbox{$M_\oplus$}}
\newcommand{\Rearth}{\mbox{$R_\oplus$}}
\newcommand{\Msun}{\mbox{$M_\odot$}}
\newcommand{\Rsun}{\mbox{$R_\odot$}}
\newcommand{\Lsun}{\mbox{$L_\odot$}}
\newcommand{\Mmoon}{\mbox{$M_{\rm moon}$}}
\newcommand{\ha}{\mbox{H$\alpha$}}
\newcommand{\hb}{\mbox{H$\beta$}}
\newcommand{\hg}{\mbox{H$\gamma$}}
\newcommand{\hd}{\mbox{H$\delta$}}
\newcommand{\lya}{\mbox{Ly$\alpha$}}
\newcommand{\lyb}{\mbox{Ly$\beta$}}
\newcommand{\df}{\mbox{d}}
\def\e0{\epsilon_0}
\def\HST{{HST}}
\def\XMM{XMM-Newton}
\def\Swift{{Swift}}
\def\degC{$^{\rm o}$C}
\def\ltsim{\raisebox{-.5ex}{$\;\stackrel{<}{\sim}\;$}}
\def\gtsim{\raisebox{-.5ex}{$\;\stackrel{>}{\sim}\;$}}
\def\hi{H\,{\sc i}}
\def\hii{H\,{\sc ii}}
\def\hei{He\,{\sc i}}
\def\heii{He\,{\sc ii}}
\def\ci{C\,{\sc i}}
\def\cii{C\,{\sc ii}}
\def\ciii{\ifmmode {\rm C}\,{\sc iii} \else C\,{\sc iii}\fi}
\def\civ{\ifmmode {\rm C}\,{\sc iv} \else C\,{\sc iv}\fi}
\def\cvi{C\,{\sc vi}}
\def\ni{N\,{\sc i}}
\def\nii{N\,{\sc ii}}
\def\niii{N\,{\sc iii}}
\def\niv{N\,{\sc iv}}
\def\nvii{N\,{\sc vii}}
\def\oi{O\,{\sc i}}
\def\oii{O\,{\sc ii}}
\def\oiii{O\,{\sc iii}}
\def\o5007{[O\,{\sc iii}]\,$\lambda5007$}
\def\oiv{O\,{\sc iv}}
\def\ov{O\,{\sc v}}
\def\ovi{O\,{\sc vi}}
\def\ovii{O\,{\sc vii}}
\def\oviii{O\,{\sc viii}}
\def\nev{Ne\,{\sc v}}
\def\mgi{Mg\,{\sc i}}
\def\mgii{Mg\,{\sc ii}}
\def\siIV{Si\,{\sc iv}}
\def\si{S\,{\sc i}}
\def\sii{S\,{\sc ii}}
\def\siii{S\,{\sc iii}}
\def\caii{Ca\,{\sc ii}}
\def\pv{P\,{\sc v}}
\def\feii{Fe\,{\sc ii}}
\def\aliii{Al\,{\sc iii}}
\def\SN{\mbox{\it S/N}}

%% Some definitions
\def\rxte{{RXTE}}
\def\suzaku{{Suzaku}}
\def\swift{{Swift}}
\def\Chandra{{Chandra}}
\def\nustar{{NuSTAR}}
\def\nicer{{NICER}}
\def\integral{{INTEGRAL}}
\def\xillver{{\tt xillver}}
\def\xillverD{{\tt xillverD}}
\def\xillverCp{{\tt xillverCp}}
\def\relxill{{\tt relxill}}
\def\relxillD{{\tt relxillD}}
\def\relxilllp{{\tt relxilllp}}
\def\relxilllpD{{\tt relxilllpD}}
\def\relxillCp{{\tt relxillCp}}
\def\relxilllpCp{{\tt relxilllpCp}}
\def\relline{{\tt relline}}
\def\nthComp{{\tt nthComp}}
\def\simplcut{{\tt simplcut}}
\def\diskbb{{\tt diskbb}}
\def\powerlaw{{\tt powerlaw}}
\def\xspec{{\tt XSPEC}}
\def\reltrans{{\tt reltrans}}
\def\reltransDCp{{\tt reltransDCp}}
